On an inverse problem of nonlinear imaging with fractional damping

This paper considers the attenuated Westervelt equation in pressure formulation. The attenuation is by various models proposed in the literature and characterised by the inclusion of non-local operators that give power law damping as opposed to the exponential of classical models. The goal is the inverse problem of recovering a spatially dependent coefficient in the equation, the parameter of nonlinearity $\kappa(x)$, in what becomes a nonlinear hyperbolic equation with nonlocal terms. The overposed measured data is a time trace taken on a subset of the domain or its boundary. We shall show injectivity of the linearised map from $\kappa$ to the overposed data used to recover it and from this basis develop and analyse Newton-type schemes for its effective recovery.

==> roots_delta.tex <==
delta=0.1
   -0.1087    6.1367
   -0.2308   12.1545
   -0.3369   18.1261
   -0.4290   24.0736
   -0.5099   30.0066
   -0.5820   35.9301
   -0.6471   41.8470
   -0.7065   47.7589
   -0.7612   53.6671
   -0.8120   59.5723

delta=0.5

   -0.5533    5.5670
   -1.2322   10.5439
   -1.8796   15.2603
   -2.4852   19.8210
   -3.0517   24.2761
   -3.5835   28.6541
   -4.0848   32.9730
   -4.5593   37.2451
   -5.0098   41.4790
   -5.4390   45.6813

delta=1
   -1.1154    4.8854
   -2.5834    8.6284
   -4.0985   11.8338
   -5.6225   14.6902
   -7.1455   17.2898
   -8.6644   19.6872
  -10.1784   21.9181
  -11.6873   24.0075
  -13.1916   25.9741
  -14.6916   27.8320

delta=2

   -2.1870    3.5207
  -19.4166    9.5005
  -28.1590   10.6607
  -36.6173   11.6192
  -44.9245   12.4450
  -53.1367   13.1759
  -61.2831   13.8348
  -69.3810   14.4372
  -77.4414   14.9936
  -85.4718   15.5119


